Smooth real-time motion planning based on a cascade dual-quaternion screw-geometry MPC

This paper investigates the tracking problem of a smooth coordinate-invariant trajectory using dual quaternion algebra. The proposed architecture consists of a cascade structure in which the outer-loop MPC performs real-time smoothing of the manipulator's end-effector twist while an inner-loop kinematic controller ensures tracking of the instantaneous desired end-effector pose. Experiments on a $7$-DoF Franka Emika Panda robotic manipulator validate the proposed method demonstrating its application to constraint the robot twists, accelerations and jerks within prescribed bounds.

==> mathematical_preliminaries.tex <==
\section{Mathematical Preliminaries\label{sec:mathematical-preliminaries}}

Dual quaternions \cite{Selig2005} are elements of the set
\begin{align*}
\mathcal{H} & \triangleq\{\quat h_{\mathcal{P}}+\dual\quat h_{\mathcal{D}}:\quat h_{\mathcal{P}},\quat h_{\mathcal{D}}\in\mathbb{H},\,\dual\neq0,\,\dual^{2}=0\},
\end{align*}

where $\mathbb{H}\triangleq\{h_{1}+\imi h_{2}+\imj h_{3}+\imk h_{4}\::\:h_{1},h_{2},h_{3},h_{4}\in\mathbb{R}\}$
is the set of quaternions, in which $\imi$, $\imj$ and $\imk$ are
imaginary units with the properties $\imi^{2}=\imj^{2}=\imk^{2}=\imi\imj\imk=-1$
\cite{Selig2005}. Addition and multiplication of dual quaternions
are analogous to their counterparts of real and complex numbers. One
must only respect the properties of the dual unit $\dual$ and imaginary
units $\imi,\imj,\imk$.

The subset $\dq{\mathcal{S}}=\left\{ \dq h\in\mathcal{H}:\norm{\dq h}=1\right\} $
of unit dual quaternions, where $\norm{\dq h}=\sqrt{\dq h\dq h^{*}}=\sqrt{\dq h^{*}\dq h}$,
with $\dq h^{*}$ being the conjugate of $\dq h$ \cite{adorno2017robot},
is used to represent poses (position and orientation) in the three-dimensional
space and form the group $\spinr$ under the multiplication operation.
Any $\dq x\in\dq{\mathcal{S}}$ can always be written as $\dq x=\quat r+\dual\left(1/2\right)\quat p\quat r$,
where $\quat p=\imi x+\imj y+\imk z$ represents the position $\left(x,y,z\right)$
and $\quat r=\cos\left(\phi/2\right)+\quat n\sin\left(\phi/2\right)$
represents a rotation, in which $\phi\in[0,2\pi)$ is the rotation
angle around the rotation axis $\quat n\in\mathbb{H}_{p}\cap\mathbb{S}^{3}$,
with $\mathbb{H}_{p}\triangleq\left\{ \quat h\in\mathbb{H}:\real{\quat h}=0\right\} $,
where $\real{h_{1}+\imi h_{2}+\imj h_{3}+\imk h_{4}}\triangleq h_{1}$,
and $\mathbb{S}^{3}=\left\{ \quat h\in\mathbb{H}:\norm{\quat h}=1\right\} $
\cite{Selig2005}.

Additionally, the logarithm of $\dq x\in\mathcal{S}$ is given by \cite{adorno2017robot}
\begin{equation}
    \log\left(\dq x\right)=\frac{\phi\quat n}{2}+\dual\frac{\quat p}{2}. \label{eq:log_dq}
\end{equation}

The set $\mathcal{H}_{p}=\left\{ \dq h\in\mathcal{H}:\real{\dq h}=0\right\} $
of pure dual quaternions is used to represent twists and wrenches,
which are represented in different coordinate systems using the adjoint
operator $\mathrm{Ad}:\dq{\mathcal{S}}\times\mathcal{H}_{p}\to\mathcal{H}_{p}$.
For instance, consider the twist $\dq{\xi}^{a}\in\mathcal{H}_{p}$
expressed in frame $\frame a$ and the unit dual quaternion $\dq x_{a}^{b}$
that represents the rigid motion from $\frame b$ to $\frame a$.
The same twist is expressed in frame $\frame b$ as

\begin{equation}
\dq{\xi}^{b}=\ad{\dq x_{a}^{b}}{\dq{\xi}^{a}}=\dq x_{a}^{b}\dq{\xi}^{a}\left(\dq x_{a}^{b}\right)^{*}.\label{eq:adj_transf}
\end{equation}
